Metric-Solver: Sliding Anchored Metric Depth Estimation from a Single Image

Accurate and generalizable metric depth estimation is crucial for various computer vision applications but remains challenging due to the diverse depth scales encountered in indoor and outdoor environments. In this paper, we introduce Metric-Solver, a novel sliding anchor-based metric depth estimation method that dynamically adapts to varying scene scales. Our approach leverages an anchor-based representation, where a reference depth serves as an anchor to separate and normalize the scene depth into two components: scaled near-field depth and tapered far-field depth. The anchor acts as a normalization factor, enabling the near-field depth to be normalized within a consistent range while mapping far-field depth smoothly toward zero. Through this approach, any depth from zero to infinity in the scene can be represented within a unified representation, effectively eliminating the need to manually account for scene scale variations. More importantly, for the same scene, the anchor can slide along the depth axis, dynamically adjusting to different depth scales. A smaller anchor provides higher resolution in the near-field, improving depth precision for closer objects while a larger anchor improves depth estimation in far regions. This adaptability enables the model to handle depth predictions at varying distances and ensure strong generalization across datasets. Our design enables a unified and adaptive depth representation across diverse environments. Extensive experiments demonstrate that Metric-Solver outperforms existing methods in both accuracy and cross-dataset generalization.

==> fig/fix_anchor.tex <==
\begin{figure}[t]
  \centering
   \includegraphics[width=1.0\linewidth]{fig/finetune.pdf}

   \caption{\textbf{Fix depth anchor}. Faced with cross-scenario, multi-scale metric depth estimation, traditional approaches typically fine-tune a pretrained model on the target domain. To achieve accurate spatial normalization, it is also necessary to manually set a maximum depth anchor, which reduces the network's generalization ability and sacrifices its capability to predict distant scenes.}
   \label{fig:onecol}
\end{figure}
